Accelerated gradient descent method for functionals of probability measures by new convexity and smoothness based on transport maps

We consider problems of minimizing functionals $\mathcal{F}$ of probability measures on the Euclidean space. To propose an accelerated gradient descent algorithm for such problems, we consider gradient flow of transport maps that give push-forward measures of an initial measure. Then we propose a deterministic accelerated algorithm by extending Nesterov's acceleration technique with momentum. This algorithm do not based on the Wasserstein geometry. Furthermore, to estimate the convergence rate of the accelerated algorithm, we introduce new convexity and smoothness for $\mathcal{F}$ based on transport maps. As a result, we can show that the accelerated algorithm converges faster than a normal gradient descent algorithm. Numerical experiments support this theoretical result.

==> sec_other_notions.tex <==
We may consider other notions of convexity and/or $L$-smoothness for functionals $\mathcal{F}$. 
We describe them below for reference. 

\subsection{Displacement convexity}
\label{sec:Lyap_2_Wass}

The displacement convexity is well-known as convesity on constant-speed geodesics. 
Because it is explained in the literature about the Wasserstein gradient flows, 
we omit its details here. 
It is consistent with the $2$-Wasserstein distance $W_{2}$. 

To estimate the convergence rate of $\mathcal{F}(\mu_{t})$ for $\mu_{t}$ given by the gradient flow, 
the Lyapunov function 
\begin{align}
\mathcal{L}_{W_{2}}(t) 
:= 
t \, (\mathcal{F}(\mu_{t}) - \mathcal{F}(\mu_{\ast})) + \frac{1}{2} \, W_{2}(\mu_{t}, \mu_{\ast})^{2}. 
\label{eq:Lyap_1}
\end{align}
By using a formula for the derivative of $W_{2}(\mu_{t}, \mu_{\ast})^{2}$ in \cite[p.~652, Thoerem 23.9]{villani2009optimal}, 
we would prove that
\begin{align}
\frac{\mathrm{d}}{\mathrm{d}t} \mathcal{L}_{W_{2}}(t) 
\leq
0
\end{align}
if $\mathcal{F}$ is displacement convex.

In the case of the accelerated gradient flow, 
we define $\mathcal{L}_{W_{2}}^{\mathrm{ac}}(t)$ by
\begin{align}
\mathcal{L}_{W_{2}}^{\mathrm{ac}}(t) 
:= 
\mathcal{A}_{W_{2}}^{\mathrm{ac}}(t)
+ 
\mathcal{B}_{W_{2}}^{\mathrm{ac}}(t), 
\end{align}
where
\begin{align}
& \mathcal{A}_{W_{2}}^{\mathrm{ac}}(t)
:= t^{r} (\mathcal{F}(\mu_{t}^{\mathrm{ac}}) - \mathcal{F}(\mu_{\ast})), 
\notag \\
& \mathcal{B}_{W_{2}}^{\mathrm{ac}}(t)
:= 
\frac{1}{2} W_{2}(Y^{\mathrm{ac}}(t, \cdot)_{\#}\mu_{0}, \mu_{\ast})^{2}. 
\notag
\end{align}
Then, 
we can deduce from \eqref{eq:diff_F_mu_t} that
\begin{align}
\frac{\mathrm{d}}{\mathrm{d}t} \mathcal{L}_{W_{2}}^{\mathrm{ac}}(t) 
=
rt^{r-1} (\mathcal{F}(\mu_{t}^{\mathrm{ac}}) - \mathcal{F}(\mu_{\ast})) + 
t^{r} \frac{\mathrm{d}}{\mathrm{d}t} \mathcal{F}(\mu_{t}^{\mathrm{ac}}) + 
\frac{\mathrm{d}}{\mathrm{d}t} \mathcal{B}_{W_{2}}^{\mathrm{ac}}(t),
\notag
\end{align}
where
\begin{align}
& t^{r} \frac{\mathrm{d}}{\mathrm{d}t} \mathcal{F}(\mu_{t}^{\mathrm{ac}})
= 
- rt^{r-1}
\int 
\Big \langle \mathcal{G}_{\mathcal{F}}[\mu_{t}^{\mathrm{ac}}](X^{\mathrm{ac}}(t,x)), \underline{X^{\mathrm{ac}}(t,x) - Y^{\mathrm{ac}}(t,x)} \Big \rangle
\, \mathrm{d}\mu_{0}(x), 
\notag \\
& \frac{\mathrm{d}}{\mathrm{d}t} \mathcal{B}_{W_{2}}^{\mathrm{ac}}(t)
= 
- rt^{r-1}
\int 
\Big \langle
\mathcal{G}_{\mathcal{F}}[\mu_{t}^{\mathrm{ac}}](X^{\mathrm{ac}}(t,x)), \ \underline{u_{t}(X^{\mathrm{ac}}(t, x)})
\Big \rangle
\, \mathrm{d}\mu_{0}(x)
\notag
\end{align}
Note that the latter is based on \cite[p.~652, Thoerem 23.9]{villani2009optimal} 
and $u_{t}$ is a certain function. 
Because of the underlined parts, 
the sum of these two may not be simplified anymore. 
As a result,
we cannot apply the same procedure as that in Section~\ref{sec:est_acc_grad_cont_flow}.
Therefore 
using $2$-Wasserstein distance would not be a good choice. 

\subsection{Average convexity and $L$-smoothess}

Here we define ``average convexity'' for functionals. 
A functional $\mathcal{F}$ is ``\emph{average convex}'' if it satisfies
\begin{align}
\mathcal{F}(T_{\#} \mu) - \mathcal{F}(S_{\#} \mu)
\geq 
\int  
\int  
\, \Big \langle \mathcal{G}_{\mathcal{F}}[S_{\#} \mu](S(x)) , \, T(y) - S(x) \Big \rangle
\, \mathrm{d}\mu(x) \, \mathrm{d}\mu(y).
\label{eq:def_aver_conv}
\end{align}
For this convexity, 
the discrepancy functional $\tilde{D}$ defined by
\begin{align}
\tilde{D}(\mu, \nu) 
:=
\int  
\int 
\| x - y \|^{2}
\, \mathrm{d}\mu(x) \, \mathrm{d}\nu(y). 
\label{eq:def_A_2}
\end{align}
is suitable for defining a Lyapunov function in place of the functional $D$ in \eqref{eq:def_discr_func}. 

For the convergence analysis of the gradient flow, 
we consider the Lyapunov function
\begin{align}
\tilde{\mathcal{L}}(t) 
:= 
t \, (\mathcal{F}(\mu_{t}) - \mathcal{F}(\mu_{\ast})) 
+
\frac{1}{2} \tilde{D}(\mu_{t}, \mu_{\ast}). 
\label{eq:def_Lyap_by_tilde_D}
\end{align}
Then, from the relation 
\begin{align}
\frac{1}{2} \tilde{D}(\mu_{t}, \mu_{\ast})
= 
\int  
\int  
\| X(t,x) - y \|^{2}
\, \mathrm{d}\mu_{0}(x) \, \mathrm{d}\mu_{\ast}(y), 
\notag
\end{align}
we can deduce that
\begin{align}
\frac{\mathrm{d}}{\mathrm{d}t} 
\left( \frac{1}{2} \tilde{D}(\mu_{t}, \mu_{\ast}) \right)
& = 
\int  
\int 
\left\langle \frac{\partial}{\partial t} X(t,x) , \, X(t,x) - y \right\rangle 
\, \mathrm{d}\mu_{0}(x) \, \mathrm{d}\mu_{\ast}(y)
\notag \\
& = 
\int 
\left\langle \frac{\partial}{\partial t} X(t,x) , \, X(t,x) - m_{\ast} \right\rangle 
\, \mathrm{d}\mu_{0}(x) 
\notag \\
& = 
- \int 
\, \Big \langle \mathcal{G}_{\mathcal{F}}[X(t, \cdot)_{\#} \mu_{0}](X(t,x)) , \, X(t,x) - m_{\ast} \Big \rangle 
\, \mathrm{d}\mu_{0}(x) 
\notag \\
& = 
- \int  
\, \Big \langle \mathcal{G}_{\mathcal{F}}[\mu_{t}](x) , \, x - m_{\ast} \Big \rangle
\, \mathrm{d}\mu_{t}(x),
\notag
\end{align}
where
\begin{align}
m_{\ast} := \int y \, \mathrm{d}\mu_{\ast}(y).
\label{eq:opt_meas_mean}
\end{align}
Then, for the Lyapunov function $\tilde{\mathcal{L}}(t)$ in~\eqref{eq:def_Lyap_by_tilde_D}, 
we have
\begin{align}
\frac{\mathrm{d}}{\mathrm{d}t} \tilde{\mathcal{L}}(t)
\leq
\mathcal{F}(\mu_{t}) - \mathcal{F}(\mu_{\ast})
-
\int  
\, \Big \langle \mathcal{G}_{\mathcal{F}}[\mu_{t}](x) , \, x - m_{\ast} \Big \rangle
\, \mathrm{d}\mu_{t}(x).
\label{eq:mysterious_convexity}
\end{align}
Then, 
if $\mathcal{F}$ is average convex in the sense of~\eqref{eq:mysterious_convexity}, 
the RHS above is non-positive 
and we can show that
$\mathcal{F}(\mu_{t}) - \mathcal{F}(\mu_{\ast}) = \mathrm{O}(1/t)$.

In the case of the accelerated gradient flow, 
we can use the Lyapunov function in~\eqref{eq:def_Lyap_by_tilde_D}
to show that 
$\mathcal{F}(\mu_{t}) - \mathcal{F}(\mu_{\ast}) = \mathrm{O}(1/t^{2})$
under the average convexity defined by~\eqref{eq:def_aver_conv}. 
However, 
we have difficulty in dealing with its discrete counterpart. 
The counterpart of $\hat{\mathcal{U}}_{n}^{\mathrm{ac}}$ in~\eqref{eq:diff_of_disc_U_NAG}
is given by
\begin{align}
\tilde{\mathcal{U}}_{n}^{\mathrm{ac}} 
& = 
\mathcal{F}(\hat{\mu}_{n+1}^{\mathrm{ac}}) - \mathcal{F}(\hat{\nu}_{n}^{\mathrm{ac}}) 
-
\int \langle \mathcal{G}_{\mathcal{F}}[\hat{\mu}_{n+1}^{\mathrm{ac}}](X_{n+1}^{\mathrm{ac}}(x)), X_{n+1}^{\mathrm{ac}}(x) - m_{\hat{\nu}_{n}^{\mathrm{ac}}} \rangle
\, \mathrm{d}\mu_{0}(x) 
\notag \\
& \phantom{= \mathcal{F}(\hat{\mu}_{n+1}^{\mathrm{ac}}) - \mathcal{F}(\hat{\nu}_{n}^{\mathrm{ac}})} \, 
-
\int \langle \mathcal{G}_{\mathcal{F}}[\hat{\mu}_{n+1}^{\mathrm{ac}}](X_{n+1}^{\mathrm{ac}}(x)), m_{\hat{\nu}_{n}^{\mathrm{ac}}} - Z_{n+1}^{\mathrm{ac}}(x) \rangle
\, \mathrm{d}\mu_{0}(x) 
\notag \\
& \leq
- \int 
\langle \mathcal{G}_{\mathcal{F}}[\hat{\mu}_{n+1}^{\mathrm{ac}}](X_{n+1}^{\mathrm{ac}}(x)), m_{\hat{\nu}_{n}^{\mathrm{ac}}} - Z_{n+1}^{\mathrm{ac}}(x) \rangle
\, \mathrm{d}\mu_{0}(x)
\notag \\
& = 
- \int \int 
\langle \mathcal{G}_{\mathcal{F}}[\hat{\mu}_{n+1}^{\mathrm{ac}}](X_{n+1}^{\mathrm{ac}}(x)), Y_{n}^{\mathrm{ac}}(y) - Z_{n+1}^{\mathrm{ac}}(x) \rangle
\, \mathrm{d}\mu_{0}(x) \, \mathrm{d}\mu_{0}(y), 
\label{eq:tilde_U_ac_bound}
\end{align}
where
\begin{align}
m_{\nu_{n}^{\mathrm{ac}}}
:=
\int y\, \mathrm{d} \hat{\nu}_{n}^{\mathrm{ac}}(y).
\notag
\end{align}
We cannot derive a counterpart of \eqref{eq:diff_of_disc_S_NAG_bound_2} from~\eqref{eq:tilde_U_ac_bound} and 
\eqref{eq:diff_of_disc_S_NAG_bound_1}. 
This is because \eqref{eq:tilde_U_ac_bound} contains the double integral with respect to $x$ and $y$. 

\begin{ex}[Example of the average convexity]
Let $W(x,y)$ be defined by
\[
W(x,y) := \| x - y \|^{2}.
\]
Then, the functional $\mathcal{F}(\mu)$ is given by
\begin{align}
\mathcal{F}(\mu)
& =
\frac{1}{2} 
\int \int 
(\| x \|^{2} - 2 \langle x, y \rangle + \| y \|^{2}) 
\, \mathrm{d}\mu(x) \, \mathrm{d}\mu(y) 
\notag \\
& = 
M_{\mu}^{(2)} - \langle m_{\mu}^{(1)} , m_{\mu}^{(1)} \rangle
\notag \\
& = 
M_{\mu}^{(2)} - \| m_{\mu}^{(1)} \|^{2}, 
\notag
\end{align}
where
\begin{align}
& M_{\mu}^{(2)} := \int \| x \|^{2} \, \mathrm{d}\mu(x) \qquad (\in \mathbf{R}), 
\notag \\
& m_{\mu}^{(1)} := \int x \, \mathrm{d}\mu(x) \qquad (\in \mathbf{R}^{d}).
\notag
\end{align}
The value $\mathcal{F}(\mu)$ is the variance of the probability measure $\mu$ and clearly $\mathcal{F}(\mu) \geq 0$.
Then, the minimization problem of $\mathcal{F}$ 
is a simple toy problem of minimizing variance of a probability measure. 

Then, 
we can estimate the value 
\begin{align}
\mathcal{F}(\mu_{t}) - \mathcal{F}(\mu_{\ast})
-
\int 
\Big \langle
\mathcal{G}_{\mathcal{F}}[\mu_{t}](x), x - m_{\ast}
\Big \rangle
\, \mathrm{d}\mu_{t}(x) 
\notag
\end{align}
as follows: 
\begin{align}
& M_{\mu_{t}}^{(2)} - \| m_{\mu_{t}}^{(1)} \|^{2} - (M_{\mu_{\ast}}^{(2)} - \| m_{\mu_{\ast}}^{(1)} \|^{2})
\notag \\
& - 
\int \int 
\langle 
2(x - y), \, 
x - m_{\mu_{\ast}}^{(1)}
\rangle
\, \mathrm{d} \mu_{t}(x) \, \mathrm{d} \mu_{t}(y) 
\notag \\
& =  
M_{\mu_{t}}^{(2)} - \| m_{\mu_{t}}^{(1)} \|^{2} - (M_{\mu_{\ast}}^{(2)} - \| m_{\mu_{\ast}}^{(1)} \|^{2})
\notag \\
& \phantom{=} \, - 2
\int \int 
(\| x \|^{2} - \langle y, x \rangle - \langle x, m_{\mu_{\ast}}^{(1)} \rangle + \langle y, m_{\mu_{\ast}}^{(1)} \rangle)
\, \mathrm{d} \mu_{t}(x) \, \mathrm{d} \mu_{t}(y)
\notag \\
& =  
M_{\mu_{t}}^{(2)} - \| m_{\mu_{t}}^{(1)} \|^{2} - (M_{\mu_{\ast}}^{(2)} - \| m_{\mu_{\ast}}^{(1)} \|^{2})
\notag \\
& \phantom{=} \, - 2
\left( 
M_{\mu_{t}}^{(2)} - \| m_{\mu_{t}}^{(1)} \|^{2}
- \langle m_{\mu_{t}}^{(1)}, m_{\mu_{\ast}}^{(1)} \rangle + \langle m_{\mu_{t}}^{(1)}, m_{\mu_{\ast}}^{(1)} \rangle
\right)
\notag \\
& =
-(M_{\mu_{t}}^{(2)} - \| m_{\mu_{t}}^{(1)} \|^{2}) - (M_{\mu_{\ast}}^{(2)} - \| m_{\mu_{\ast}}^{(1)} \|^{2})
\notag \\
& \leq 0.
\notag
\end{align}
The last inequality follows from the fact that $M_{\mu}^{(2)} - \| m_{\mu}^{(1)} \|^{2} \geq 0$ for any $\mu$. 
Therefore $\mathcal{F}$ is average convex. 
Then, we can apply the convergence results in 
Section~\ref{sec:grad_Lyap_2}
to this $\mathcal{F}$.
\end{ex}

However, 
the average convexity defined by~\eqref{eq:def_aver_conv}
would not be useful 
because 
the typical functions considered in Section~\ref{sec:new_conv_and_L_smooth} would not average convex. 

